Cascaded channel pruning using hierarchical self-distillation

In this paper, we propose an approach for filter-level pruning with hierarchical knowledge distillation based on the teacher, teaching-assistant, and student framework. Our method makes use of teaching assistants at intermediate pruning levels that share the same architecture and weights as the target student. We propose to prune each model independently using the gradient information from its corresponding teacher. By considering the relative sizes of each student-teacher pair, this formulation provides a natural trade-off between the capacity gap for knowledge distillation and the bias of the filter saliency updates. Our results show improvements in the attainable accuracy and model compression across the CIFAR10 and ImageNet classification tasks using the VGG16and ResNet50 architectures. We provide an extensive evaluation that demonstrates the benefits of using a varying number of teaching assistant models at different sizes.

==> results/layer_pruning_bar_chart_vgg16.tex <==
\begin{tikzpicture}[
    every axis/.style={
        ybar stacked,
        ymin=0.0,ymax=1.0,
        xmin=1,xmax=10,
        bar width=8pt
    }
]

\begin{axis}[
    axis y line*=left,
    axis x line*=bottom,
    ylabel=
]
\addplot[
    fill opacity=0.5,
    draw opacity=0.5,
    fill=fill_red,
    draw=red
] coordinates
{(1, 0.1) (2, 0.1) (3, 0.1) (4, 0.1) (5, 0.1) (6, 0.1) (7, 0.1) (7, 0.1) (8, 0.1) (9, 0.1) (10, 0.1)};
\addplot+[
    fill opacity=0.5,
    draw opacity=0.5,
    fill=fill_blue,
    draw=red
] coordinates
{(1, 0.1) (2, 0.1) (3, 0.1) (4, 0.1) (5, 0.1) (6, 0.1) (7, 0.1) (7, 0.1) (8, 0.1) (9, 0.1) (10, 0.1)};
\addplot+[
    fill opacity=0.5,
    draw opacity=0.5,
    fill=fill_yellow,
    draw=red
] coordinates
{(1, 0.1) (2, 0.1) (3, 0.1) (4, 0.1) (5, 0.1) (6, 0.1) (7, 0.1) (7, 0.1) (8, 0.1) (9, 0.1) (10, 0.1)};
\end{axis}

\end{tikzpicture}

==> results/resnet50.tex <==
\begin{table*}[t!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        Block \# & $w \times h$ & \#Filters & FLOPs  & Params \\
        \hline
        & $224 \times 224$ & $64$ & 118M & 0.01M \\
        
        % Identity block: 1x1 F1, 3x3 F2, 1x1 F3
        % Conv block: 1x1 F1, 3x3 F2, 1x1 F3 + 1x1 F3

        \hline
        0 & $56 \times 56$ & $[64, 64, 256]$ & 231M & 0.07M \\
        1 & $56 \times 56$ & $[64, 64, 256]$ & 218M & 0.07M \\
        2 & $56 \times 56$ & $[64, 64, 256]$ & 218M & 0.07M \\
        \hline
        
        3 & $56 \times 56$ & $[128, 128, 512]$ & 295M & 0.38M \\
        4 & $28 \times 28$ & $[128, 128, 512]$ & 218M & 0.28M \\
        5 & $28 \times 28$ & $[128, 128, 512]$ & 218M & 0.28M \\
        6 & $28 \times 28$ & $[128, 128, 512]$ & 218M & 0.28M \\
        \hline
        
        \hline
        7 & $28 \times 28$ & $[256, 256, 1024]$ & 295M & 1.51M \\
        8 & $14 \times 14$ & $[256, 256, 1024]$ & 218M & 1.11M \\
        9 & $14 \times 14$ & $[256, 256, 1024]$ & 218M & 1.11M \\
        10 & $14 \times 14$ & $[256, 256, 1024]$ & 218M & 1.11M \\
        11 & $14 \times 14$ & $[256, 256, 1024]$ & 218M & 1.11M \\
        12 & $14 \times 14$ & $[256, 256, 1024]$ & 218M & 1.11M \\
        \hline
        
        13 & $14 \times 14$ & $[512, 512, 2048]$ & 295M & 6.03M \\
        14 & $7 \times 7$ & $[512, 512, 2048]$ & 218M & 4.46M \\
        15 & $7 \times 7$ & $[512, 512, 2048]$ & 218M & 4.46M \\
        \hline
        
        & $1 \times 1$ & $1000$ & 2.05M & 2.05M \\
        % \multicolumn{5}{c}{} \\
        \hline
        \multicolumn{3}{|c|}{Total:} & 3.85B & 25.5M \\
        \hline
        
    \end{tabular}%
    \caption{Performance statistics for the ResNet50 architecture on the ImageNet2012 dataset.}
    \label{table:resnet50_statistics}
\end{table*}

==> tables/faster_rcnn.tex <==
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        Backbone & Params & FLOPs  & maP @ 0.5 & maP @ [0.5, 0.95] \\
        \hline
        Original & 3.89M & 495M & 74.10\% \\
        \hline
        TDN-0.1 & - & - & \% \\
        \hline
        TDN-0.2 & - & - & 73.81\% \\
        \hline
        % TDN-0.6 & - & - & \sidenote{69.91}\% \\
        TDN-0.5 & 1.78M & 163M & \% \\
        \hline
    \end{tabular}%
    \caption{-}
    \label{table:faster_rcnn_results}
\end{table}
